Plasma Spray Process Parameters Configuration using Sample-efficient Batch Bayesian Optimization

Recent work has shown constrained Bayesian optimization to be a powerful technique for the optimization of industrial processes. In complex manufacturing processes, the possibility to run extensive sequences of experiments with the goal of finding good process parameters is severely limited by the time required for quality evaluation of the produced parts. To accelerate the process parameter optimization, we introduce a parallel acquisition procedure tailored on the process characteristics. We further propose an algorithm that adapts to equipment status to improve run-to-run reproducibility. We validate our optimization method numerically and experimentally, and demonstrate that it can efficiently find input parameters that produce the desired outcome and minimize the process cost.

==> Reviews/Answer_to_reviewers.tex <==

\textbf{\large Reply to Reviewer 1:}\\\\
We would like to appreciate the reviewer for their evaluation as well as their comments and suggestions on improving the quality of the manuscript.\\  


%----------------------------------------------------------------------

\textbf{Comment 1:}
First off, I love the application of Bayesian optimization (or, more
generally, intelligent design of experiments) to another new
field/topic.  I think that the authors have worked to achieve the
hardest part of the adaptation process required to leverage advanced
modifications of BO in previously uncharted territory. ...I would like to start this by saying that I enjoy the novelty of your
acquisition function.

\textbf{Reply:}
We thank the reviewer for the feedback. 
 



\textbf{Comment 2:} 

It is not obvious to me what this paper is trying to achieve.  On
one hand, I think the authors argue that they are trying to build a
Gaussian process modeling strategy specific to their problem, as well
as an acquisition function better suited to their specific form of
constrained BO.  That is good, I like that -- but then the strategy
that you used and the results of your paper are only relevant to your
exact problem (which is so secretive that you couldn't even explain
completely what it is). 

\textbf{Reply:}


\textbf{Comment 3:}  I have no perspective of
the significance of the modeling results presented in Figures 2 & 3,
nor the BO results presented in Figures 4 & 5.	Frankly, I don't know
what fraction of the RA-L audience is going to understand how difficult
it is to achieve your goal to "find combinations of inputs producing
coatings with microhardness ranging between 635HV and 675HV and
porosity between 6% and 8.2% while minimizing the gun stress index." 
And you do not present any competing methods to provide a frame of
reference for readers.

I can be okay with the idea that the application is just a motivation
and your real contribution is the algorithm.  But I see two fundamental
problems with how you have executed on this front.  First, the
algorithm is never compared against any alternatives, or even on any
problems that anyone else in the world can run (given your
confidentiality).  How can the significance of your work be judged in
such a vacuum?	Second, you have done a significant amount of work to
develop modeling strategies which are, possibly, only relevant for this
specific application.  If you want to argue that there is an
algorithmic contribution, don't you need to test this algorithm more
broadly and see when it performs well and when it does not?

Essentially, my main problem is that this article wants to focus on a
specific application but is trying to present a result as being more
general than is demonstrated.  Either a number of more general tests
need to be run to make an actual statement about your algorithm, or you
should publish this in a forum where people can understand your
application, and then more specifically explain the significance of
this previously unachieved performance.

\textbf{Reply:}

\textbf{Comment 4 (or 4&5):}  The results in Figure 2 seem a bit troubling to me.	First, you said
that you created 86 pieces of data for your training set and 23 pieces
of data for your validation set.  When I look at the Porosity graph, I
count only 15 red squares.  Am I misunderstanding where the 23 is being
used, or are there just some squares that happen to lie exactly on top
of each other?	If there are, that seems a bit odd, right, given your
statement in Table II about how much noise is affecting the
accumulation of data?

\textbf{Reply:}


\textbf{Comment 5:} Beyond that, I am very concerned about the distribution of the
Validation values relative to the Training values.  When I think about
the training/validation split in surrogate modeling, I think that the
goal is for the training and validation sets to somehow be drawn from
the same distribution.	The fact that the red squares seem to occupy
only a fraction of the region that the blue dots occupy makes me
worried that they do not belong to the same distribution.  As a result,
it makes me somewhat concerned about how effective these GP models are,
and in turn how much your algorithm actually relies on them (assuming
the algorithm is performaing well).

Your strategy for creating this validation set was arbitrary, and not
at all reproducible (given the expertise required), so this is part of
my concern about suggesting a signficant algorithmic novelty in this
article.

\textbf{Reply:}


\textbf{Comment 6:}
Along these lines, I worry about this voltage discussion.  First,
Figure 3 seems to present a bizarre disconnect between the training and
validation data; why did you use totally different methods to create
the training and validation datasets?  Why not use the exact same
strategy for both?  Second I can read the Section IV-C and somewhat
understand how you are incorporating voltage, but not really. And it
should not matter if the focus is on the algorithmic side (since this
strategy would not be applicable in any other settings).  The comment
"voltage cannot be ... optimized" feels false as well.	If I
understand, voltage is a function of your tunable parameters.  How
would optimizing it be any different than optimizing any other
black-box function (which is what BO is built to do)?


\textbf{Reply:}


\textbf{Comment 7:} In your abstract you claim "We ... propose an algorithm that adapts
to real-time process measurements to improve reproducibility."	I do
not feel that you have done that anywhere in the paper.  I do not even
really know what reproducibility means in this context?  Do you mean
that if you run the exact same parameters your gun will work exactly
the same way?  I do not think that is true -- isn't that what Table II
is meant to demonstrate?  Do you mean reproduciblity of the BO?  In
general, BO is reproducible if run in a deterministic fashion, but
generally is meant to be stochastic (and will not be reproducible).  I
think you either need to retract this claim or better explain your
definition of reproduciblity.

\textbf{Reply:}

\textbf{Comment 8:} Your acquisition function and BO involves some interesting elements.
 First, it seems like you are treating S(x) as though it were free to
compute.  If this is the case, it should probably be stated (since that
is the opposite of the standard assumption).

Another place where the algorithmic novelty is insufficiently
demonstrated is in section IV-A.  "In preliminary experiments, we
observed that acquisition procedures such as the one presented in [12]
were too aggressive, while an approach focusing on FIP only led to
excessively conservative exploration."	You just say this, and that's
it.  In my opinion, if you are going to make this claim then you need
to present results to that effect.  You can do that for the situation
that you are working in, or on a manufactured problem (which would
probably be preferable).  But without that, you are just saying
something that the audience cannot verify, or even really place in
their own context.

I would also like to see more analysis of your acquisition function in
action, including with consideration of the pi value that appears (but
for which we are not really given guidance on choosing).  I worry a bit
about the fact that you fix 20000 points rather than conducting an
actual optimization over the entire space, but I don't think that's the
end of the world.

\textbf{Reply:}


\textbf{Comment 9:} The parameters that you were studying were all discrete: if I
correctly understood section V-A, 6 parameters with 3 values and 2
parameters with 2 values, for a total of 2916 possible parametrizations
of the experimental setup.  Is this correct?  If so, what are the 20000
candidates you describe creating in section IV-C?  Shouldn't there only
be 2916?  If you mean to work in a continuous space, then when was your
training/validation set created using a discrete domain?

\textbf{Reply:}


\textbf{Comment 10:} I do not understand what is meant to be demonstrated in Figure 5. 
Why would you plot anything related to the "first optimization batch"? 
Why would that be relevant?  Wouldn't you somehow want to either plot
all of the feasible results or, simply, all of the results?  And why do
you provide the 95% prediction confidence?  What is that meant to
convey?  Is that a function of your models that you have built?  Aren't
we actually taking real values from the gun at this point?  Why does it
matter what your model says for a location where we actually have data?

And actually, at this point, I have a more confusing question -- did
you run this for only a single BO iteration?  There does not seem to be
any explanation of the actual results of your BO process, only the
first batch (of which you cut one because you felt like it).  What
epsilon did you use for these experiments that led you to conduct only
a single iteration?

\textbf{Reply:}


\textbf{Comment 11:}
I also do not understand what Figure 4 is.  Was this an actual
experiment that was run?  Or is this just a demonstration of what
something should look like?  If this is an actual experiment, why was
it run to 4 batches when the other experiment was run for only a single
batch?


\textbf{Reply:}


==> Reviews_summary.tex <==
Major issues:
Major points:


- Experiments provide no comparisons against baseline methods. The modelling component of the proposed framework is assessed in terms of predictive power against real data. The optimisation component, however, an essential part of the paper's main contribution is not compared against other methods. Therefore, it is hard to judge whether the proposed BO framework offers real performance improvements against existing out-of-the-box constrained BO methods (e.g., [12]).
One could argue that experimental comparisons using the real APS system are too expensive to run, so that the results in Sec. VI-B are still acceptable. However, the numerical experiments in Sec. VI-A were performed using a neural network oracle, which should much cheaper to evaluate, allowing for comparisons against other BO methods as baselines.

- the strategy that you used and the results of your paper are only relevant to your exact problem (which is so secretive that you couldn't even explain completely what it is).  That can be fine, but I have no perspective of the significance of the modeling results presented in Figures 2 & 3, nor the BO results presented in Figures 4 & 5.	Frankly, I don't know what fraction of the RA-L audience is going to understand how difficult it is to achieve your goal to "find combinations of inputs producing coatings with microhardness ranging between 635HV and 675HV and porosity between 6\% and 8.2\% while minimizing the gun stress index."  And you do not present any competing methods to provide a frame of reference for readers.
- First, the algorithm is never compared against any alternatives, or even on any problems that anyone else in the world can run (given your confidentiality).  How can the significance of your work be judged in such a vacuum? Second, you have done a significant amount of work to develop modeling strategies which are, possibly, only relevant for this specific application.  If you want to argue that there is an algorithmic contribution, don't you need to test this algorithm more broadly and see when it performs well and when it does not?
Essentially, my main problem is that this article wants to focus on a specific application but is trying to present a result as being more general than is demonstrated.  Either a number of more general tests need to be run to make an actual statement about your algorithm, or you should publish this in a forum where people can understand your application, and then more specifically explain the significance of this previously unachieved performance.
- Another place where the algorithmic novelty is insufficiently demonstrated is in section IV-A.  "In preliminary experiments, we observed that acquisition procedures such as the one presented in [12] were too aggressive, while an approach focusing on FIP only led to excessively conservative exploration."	You just say this, and that's
it.  In my opinion, if you are going to make this claim then you need to present results to that effect.  You can do that for the situation that you are working in, or on a manufactured problem (which would probably be preferable).  But without that, you are just saying something that the audience cannot verify, or even really place in their own context.

- Beyond that, I am very concerned about the distribution of the Validation values relative to the Training values.  When I think about the training/validation split in surrogate modeling, I think that the goal is for the training and validation sets to somehow be drawn from the same distribution.	The fact that the red squares seem to occupy only a fraction of the region that the blue dots occupy makes me worried that they do not belong to the same distribution.  As a result, it makes me somewhat concerned about how effective these GP models are, and in turn how much your algorithm actually relies on them (assuming the algorithm is performaing well).
Your strategy for creating this validation set was arbitrary, and not at all reproducible (given the expertise required), so this is part of my concern about suggesting a signficant algorithmic novelty in this article.

- I would also like to see more analysis of your acquisition function in action, including with consideration of the pi value that appears (but for which we are not really given guidance on choosing).




Relevant observations:

- The results in Figure 2 seem a bit troubling to me. First, you said that you created 86 pieces of data for your training set and 23 pieces of data for your validation set.  When I look at the Porosity graph, I count only 15 red squares.  Am I misunderstanding where the 23 is being used, or are there just some squares that happen to lie exactly on top of each other?	If there are, that seems a bit odd, right, given your statement in Table II about how much noise is affecting the accumulation of data?

- There is some missing detail about the modelling of the constraints. Are each of the constraints (c_1 and c_2) modelled with an independent GP? Or are they jointly modelled by a vector-valued GP?

- There is a lack of the explanation of whether collected training data set are able to cover regression feature-space effectively? If it is ineffective, the generalization ability is limited without high accuracy of prediction for those sufficient distant data points.

- In the subsection of Modeling Validation, an explanation of why the selected five combinations have the highest confidence should be provided. 

- Along these lines, I worry about this voltage discussion.  First, Figure 3 seems to present a bizarre disconnect between the training and validation data; why did you use totally different methods to create the training and validation datasets?  Why not use the exact same strategy for both?  Second I can read the Section IV-C and somewhat understand how you are incorporating voltage, but not really. And it should not matter if the focus is on the algorithmic side (since this strategy would not be applicable in any other settings).  The comment "voltage cannot be ... optimized" feels false as well.	If I understand, voltage is a function of your tunable parameters. How would optimizing it be any different than optimizing any other black-box function (which is what BO is built to do)?

- In your abstract you claim "We ... propose an algorithm that adapts to real-time process measurements to improve reproducibility."	I do not feel that you have done that anywhere in the paper.  I do not even really know what reproducibility means in this context?  Do you mean that if you run the exact same parameters your gun will work exactly the same way?  I do not think that is true -- isn't that what Table II is meant to demonstrate?  Do you mean reproduciblity of the BO?  In general, BO is reproducible if run in a deterministic fashion, but generally is meant to be stochastic (and will not be reproducible).  I think you either need to retract this claim or better explain your definition of reproduciblity.

- Your acquisition function and BO involves some interesting elements. First, it seems like you are treating S(x) as though it were free to compute.  If this is the case, it should probably be stated (since that is the opposite of the standard assumption).




Not too relevant observations:

- Gaussian process regression (GPR) is used to predict coating properties, its high computational complexity of both large data points and high dimension (using all variables in Section of Method) limits the real-time application. An explanation of your tractable computation power should be provided.

- I worry a bit about the fact that you fix 20000 points rather than conducting an actual optimization over the entire space, but I don't think that's the end of the world.

- The parameters that you were studying were all discrete: if I correctly understood section V-A, 6 parameters with 3 values and 2 parameters with 2 values, for a total of 2916 possible parametrizations of the experimental setup.  Is this correct?  If so, what are the 20000 candidates you describe creating in section IV-C?  Shouldn't there only be 2916?  If you mean to work in a continuous space, then when was your training/validation set created using a discrete domain?

- I do not understand what is meant to be demonstrated in Figure 5. Why would you plot anything related to the "first optimization batch"? Why would that be relevant?  Wouldn't you somehow want to either plot all of the feasible results or, simply, all of the results?  And why do you provide the 95\% prediction confidence?  What is that meant to convey?  Is that a function of your models that you have built?  Aren't we actually taking real values from the gun at this point?  Why does it matter what your model says for a location where we actually have data?
And actually, at this point, I have a more confusing question -- did you run this for only a single BO iteration? There does not seem to be any explanation of the actual results of your BO process, only the first batch (of which you cut one because you felt like it).  What epsilon did you use for these experiments that led you to conduct only a single iteration?
I also do not understand what Figure 4 is.  Was this an actual experiment that was run?  Or is this just a demonstration of what something should look like?  If this is an actual experiment, why was it run to 4 batches when the other experiment was run for only a single batch? 

